Machine Learning for Online Algorithm Selection under Censored Feedback

In online algorithm selection (OAS), instances of an algorithmic problem class are presented to an agent one after another, and the agent has to quickly select a presumably best algorithm from a fixed set of candidate algorithms. For decision problems such as satisfiability (SAT), quality typically refers to the algorithm's runtime. As the latter is known to exhibit a heavy-tail distribution, an algorithm is normally stopped when exceeding a predefined upper time limit. As a consequence, machine learning methods used to optimize an algorithm selection strategy in a data-driven manner need to deal with right-censored samples, a problem that has received little attention in the literature so far. In this work, we revisit multi-armed bandit algorithms for OAS and discuss their capability of dealing with the problem. Moreover, we adapt them towards runtime-oriented losses, allowing for partially censored data while keeping a space- and time-complexity independent of the time horizon. In an extensive experimental evaluation on an adapted version of the ASlib benchmark, we demonstrate that theoretically well-founded methods based on Thompson sampling perform specifically strong and improve in comparison to existing methods.

==> prediction_time_analysis_text.tex <==
\section{Detailed Prediction Time Analyses}\label{sec:app_prediction_time_analysis}
Table \ref{tab:full_prediction_times} shows the average prediction time per instance and the corresponding standard deviation of each approach for the different scenarios. The best value for each scenario is printed in bold, whereas the second best is underlined. Recall that by prediction time, we mean the time an approach requires for making a single prediction and updating its model with the corresponding feedback. As already concluded in the main paper, the Degroote variants are much slower than all true online algorithms. As expected, the LinUCB variants are faster than the Thompson variants, which include more sophisticated computations, in particular sampling from a multivariate normal distribution. We should note that the exact times of the LinUCB variants have to be treated with care. As they are already quite small, they are very susceptible to noise induced by the task scheduler of the operating system over which we have no control. Hence, a direct comparison between the LinUCB variants in terms of prediction time should not be made. Nevertheless, it is clear that they are much faster than the Thompson variants and Degroote approaches.

\begin{table}[ht]
    \centering
    \rotatebox{270}{
    \resizebox*{0.9\textheight}{!}{
        \input{tables/prediction_times}
    }
    }
    \caption{Average prediction time per instance and the corresponding standard deviation of each approach for the different scenarios. \label{tab:full_prediction_times}}
\end{table}

As Table \ref{tab:full_prediction_times} does not properly convey the disadvantage of the Degroote variants, i.e., that their time-complexity depends on the time-horizon, Figure \ref{fig:app_runtime} shows the prediction time of the most sophisticated variants presented in this work for the different scenarios over the course of the time, i.e., over multiple instances. The times are averaged over ten repetitions and the shaded areas indicate the corresponding standard deviation. Not only can we clearly see that the Degroote variants (based on the random forest) require more time than our approaches, but also that their prediction time becomes longer the more instances they have seen (as expected). However, depending on the scenario (cf. Figure \ref{fig:app_runtime_sat11-indu}), it seems that the time to train the underlying random forest of the Degroote variants stagnates at some point yielding a less steep slope at some point. This is most likely caused by the underlying random forest, whose maximum depth has been reached and hence, the splits remain the same in large parts. Nevertheless, both the time- and space-complexity of the corresponding approaches does still increase, although less extreme. In contrast to that, all of our approaches show a (noisy) constant prediction time, which only depends on the number of features of the corresponding scenario. A careful reader might observe the increase of prediction time of our approaches, especially the Thompson variants, at the start of each scenario, i.e., for the first couple of instances. This is mainly caused by two factors: First, the matrices $(A_{t,a})_{a\in \algorithms}$ have to be inverted, which is easier during the first steps of the algorithm as these matrices are very similar to the identity matrix (the initialization). Similarly, sampling from the multivariate Gaussian distribution based on the current weight vector and the corresponding covariance matrix is easier during the first steps.

Moreover, one can verify that our approaches require more prediction time on scenarios with more features such as SAT03-16\_INDU as expected. This scenario is in particular interesting as the Thompson variant requires more prediction time than the Degroote variants at the beginning, i.e., for the first $\approx 1000$ instances, but is overtaken by the Degroote variants eventually as they increase in terms of prediction time in the long run.

Lastly, we can see that the UCB variant of the Degroote approach often features longer prediction time than the epsilon-greedy variant. This is the case as the computation of the standard deviation using the Jackknife method is much more computationally demanding than the epsilon-based selection.

\input{img/runtime_figures.tex}
